Sampling and Uniqueness Sets in Graphon Signal Processing

In this work, we study the properties of sampling sets on families of large graphs by leveraging the theory of graphons and graph limits. To this end, we extend to graphon signals the notion of removable and uniqueness sets, which was developed originally for the analysis of signals on graphs. We state the formal definition of a $\Lambda-$removable set and conditions under which a bandlimited graphon signal can be represented in a unique way when its samples are obtained from the complement of a given $\Lambda-$removable set in the graphon. By leveraging such results we show that graphon representations of graphs and graph signals can be used as a common framework to compare sampling sets between graphs with different numbers of nodes and edges, and different node labelings. Additionally, given a sequence of graphs that converges to a graphon, we show that the sequences of sampling sets whose graphon representation is identical in $[0,1]$ are convergent as well. We exploit the convergence results to provide an algorithm that obtains approximately close to optimal sampling sets. Performing a set of numerical experiments, we evaluate the quality of these sampling sets. Our results open the door for the efficient computation of optimal sampling sets in graphs of large size.

==> source_figs/fig1/fig_1_tikz_source.tex <==
%!TEX root = fig_1_standalone.tex





\PreviewEnvironment{tikzpicture}
\setlength\PreviewBorder{5pt}%








%-----------------------
%------ Scale ----------
%-----------------------

\def\scale{1}
\def\unit{ \scale cm}

% Scale for the images
\def \imgscale{0.05}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  COLORS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{my_blue}{rgb}{0.0314, 0.3569, 1.0000}

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}




%\def\axisdefaultwidth{5cm}
%\def\axisdefaultheight{5cm}
%\pgfplotsset{every axis/.style={scale only axis}}





\def\grid_step{0.883cm} % Step of the grid
\def\myplotdimx{6cm}
\def\myplotdimy{6cm}
\def\my_gap_inter_plots{1.3cm}





\begin{tikzpicture}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% FIRST ROW WITH GRAPHONS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% axis style, ticks, etc
\pgfplotsset{every axis/.append style={
		%axis x line=middle,    % put the x axis in the middle
		%axis y line=middle,    % put the y axis in the middle
		%axis line style={<->}, % arrows on the axis
		%xlabel={$x$},          % default put x on x-axis
		%ylabel={$y$},          % default put y on y-axis
		title style={font=\Large},
		label style={font=\Large},
		tick label style={font=\large}  
	}}


%%-------------------------------------------------------
%%--------------- Graphon: Regular Grid Integral ---------------
%%-------------------------------------------------------

% Graphon 

	\begin{axis}[name=plot1,view={0}{90},
	    domain=0:1pt,
	    xmin=0, xmax=1pt,
	    ymin=0, ymax=1pt,
		xlabel=$x$,
		ylabel=$y$,
		title= {$W(x,y)$},
		width=\myplotdimx,
		height=\myplotdimy,
		]
		\addplot3[patch,shader=interp, colormap/viridis] {x*y};
	\end{axis}
	
	
%---------------  Regular Grid --------------

\draw[step=\grid_step, thin,color=my_cp4_col1] (0,0) grid (\grid_step*5,\grid_step*5);

%---------  Highlighting the subdomain --------

\fill[my_cp4_col1, opacity=0.7] (2*\grid_step,2*\grid_step) rectangle (3*\grid_step,3*\grid_step);


	
	
	
		
%%---------------------------------------------------
%%------------2 Graphon: Irregular Grid Integral -------------
%%---------------------------------------------------

% Graphon	

	\begin{axis}[name=plot2,at={($(plot1.south east)+(\my_gap_inter_plots,0)$)},view={0}{90}, anchor = south west,
	    domain=0:1pt,
	    xmin=0, xmax=1pt,
	    ymin=0, ymax=1pt,
	    xlabel=$x$,
	    ylabel=$y$,
	    title= {$W(x,y)$},
		width=\myplotdimx,
		height=\myplotdimy,
	    ]
	    \addplot3[patch,shader=interp, colormap/viridis] {x*y};
	\end{axis}

%---------------  Irregular Grid --------------

% Vertical lines
\path (plot2.south west)++(0.5*\grid_step,0)  coordinate (p1);
\path (plot2.south west)++(0.5*\grid_step,5*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot2.south west)++(2.3*\grid_step,0)  coordinate (p1);
\path (plot2.south west)++(2.3*\grid_step,5*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;
	
\path (plot2.south west)++(2.9*\grid_step,0)  coordinate (p1);
\path (plot2.south west)++(2.9*\grid_step,5*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;	
	
\path (plot2.south west)++(3.9*\grid_step,0)  coordinate (p1);
\path (plot2.south west)++(3.9*\grid_step,5*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;		
	
% Horizontal lines

\path (plot2.south west)++(0,0.8*\grid_step)  coordinate (p1);
\path (plot2.south west)++(5*\grid_step,0.8*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot2.south west)++(0,2*\grid_step)  coordinate (p1);
\path (plot2.south west)++(5*\grid_step,2*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot2.south west)++(0,2.2*\grid_step)  coordinate (p1);
\path (plot2.south west)++(5*\grid_step,2.2*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot2.south west)++(0,4.3*\grid_step)  coordinate (p1);
\path (plot2.south west)++(5*\grid_step,4.3*\grid_step) coordinate (p2);
\draw[my_cp4_col1, thin] (p1) -- (p2) ;

%--------------- Highlight sub-domain -------------

\path (plot2.south west)++(2.3*\grid_step,2*\grid_step)   coordinate (p1);
\path (plot2.south west)++(2.9*\grid_step,2.2*\grid_step)  coordinate (p2);
\fill[my_cp4_col1,opacity=0.7] (p1) rectangle (p2);
	
	
	
	
	
	
	
%%---------------------------------------------------
%%------------ Graphon: Irregular Sampling ----------------
%%---------------------------------------------------	
	
% Graphon	
\begin{axis}[name=plot3,at={($(plot2.south east)+(\my_gap_inter_plots,0)$)},view={0}{90}, anchor = south west,
domain=0:1pt,
xmin=0, xmax=1pt,
ymin=0, ymax=1pt,
xlabel=$x$,
ylabel=$y$,
title= {$W(x,y)$},
		width=\myplotdimx,
		height=\myplotdimy,
]
\addplot3[patch,shader=interp, colormap/viridis] {x*y};
\end{axis}
	
	
%---------------  Irregular Grid --------------

% Vertical lines

\path (plot3.south west)++(0.3*\grid_step,0)  coordinate (p1);
\path (plot3.south west)++(0.3*\grid_step,5*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot3.south west)++(2.3*\grid_step,0)  coordinate (p1);
\path (plot3.south west)++(2.3*\grid_step,5*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot3.south west)++(3.1*\grid_step,0)  coordinate (p1);
\path (plot3.south west)++(3.1*\grid_step,5*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;	

\path (plot3.south west)++(3.7*\grid_step,0)  coordinate (p1);
\path (plot3.south west)++(3.7*\grid_step,5*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;		

% Horizontal lines

\path (plot3.south west)++(0,0.7*\grid_step)  coordinate (p1);
\path (plot3.south west)++(5*\grid_step,0.7*\grid_step) coordinate (p2);
\draw[dashed,my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot3.south west)++(0,1.7*\grid_step)  coordinate (p1);
\path (plot3.south west)++(5*\grid_step,1.7*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot3.south west)++(0,2.3*\grid_step)  coordinate (p1);
\path (plot3.south west)++(5*\grid_step,2.3*\grid_step) coordinate (p2);
\draw[dashed, my_cp4_col1, thin] (p1) -- (p2) ;

\path (plot3.south west)++(0,4.3*\grid_step)  coordinate (p1);
\path (plot3.south west)++(5*\grid_step,4.3*\grid_step) coordinate (p2);
\draw[dashed,my_cp4_col1, thin] (p1) -- (p2) ;

%--------------- Highlight sub-domain -------------

\path (plot3.south west)++(2.3*\grid_step,1.7*\grid_step)  coordinate (p1);
\filldraw[my_cp4_col1,opacity=0.7] (p1) circle (0.15cm);
	
	
	
	
	
	
%%-------------------------------------------------------------
%%------------ Equations calculating adjacency from Graphons -----------
%%-------------------------------------------------------------		
	
%------ Integral symbol calculating area --------

\path (plot1.south east)+(0,-1.2*\my_gap_inter_plots) coordinate (c1);
\node (int1) at (c1)  [font=\Large]  {$ \mathbf{S}(3,3) = \displaystyle \iint_{I_3 \times I_3} W(x,y)dxdy$};

% Arrow  1
\path (plot1.south west)+(2.5*\grid_step,2.5*\grid_step) coordinate (c2);
\draw [-stealth,thick, opacity=0.7,color=my_cp4_col4,dashed] (c1) -- (c2) node[midway,above,rotate=0,color=black] {$$};

% Arrow  2
\path (plot2.south west)+(2.5*\grid_step,2.1*\grid_step) coordinate (c2);
\draw [-stealth,thick, opacity=0.7,color=my_cp4_col4,dashed] (c1) -- (c2) node[midway,above,rotate=0,color=black] {$$};


%------ Symbol taking sampling value to matrix --------

\path (plot3.south)+(0,-1.2*\my_gap_inter_plots) coordinate (c1);
\node (samp1) at (c1) [font=\Large] {$\displaystyle \mathbf{S}(2,2) = W(x_2,y_2)dxdy$};

% Arrow  3
\path (plot2.south west)+(1.5*\grid_step,1.5*\grid_step) coordinate (c2);
\draw [-stealth,thick, opacity=0.7,color=my_cp4_col4,dashed] (c1) -- (p1.north) node[midway,above,rotate=0,color=black] {$$};










	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SECOND ROW WITH GRAPHS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
\def\mynodesize{20};

%%------------------------------------------
%%------------ Graph 1 -----------------------
%%------------------------------------------

% Offset to locate the graphs

\path (plot1.south)+(0, -4*\my_gap_inter_plots)  coordinate (caux1);	


%   coordinates to plot the graph
%   1.0000    0.3090    -0.8090   -0.8090    0.3090    1.0000
%   0             0.9511    0.5878     -0.5878   -0.9511   -0.0000


%----------- Drawing the nodes ------------

\SetDefaultUnit{pt}

% radius underlying circle = 2cm
\def\myrad{2cm};

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=1, opacity=0.7,fontsize=\Large]{A}

\path (caux1)++(0.3090*\myrad ,0.9511*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=2, opacity=0.7,fontsize=\Large]{B}

\path (caux1)++(-0.8090*\myrad , 0.5878*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=3, opacity=0.7,fontsize=\Large]{C}

\path (caux1)++(-0.8090*\myrad,-0.5878*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=4, opacity=0.7,fontsize=\Large]{D}

\path (caux1)++(0.3090*\myrad,-0.9511*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=5, opacity=0.7,fontsize=\Large]{E}

%----------- Drawing the Edges  ------------

\Edge[loopposition=0,loopsize=.5cm,lw=1,color=my_cp5_col2,opacity=0.7](A)(A);
\Edge[loopposition=72,loopsize=.5cm,lw=1,color=my_cp5_col2,opacity=0.7](B)(B);
\Edge[loopposition=144,loopsize=.5cm,lw=1,color=my_cp5_col2,opacity=0.7](C)(C);
\Edge[loopposition=216,loopsize=.5cm,lw=1,color=my_cp5_col2,opacity=0.7](D)(D);
\Edge[loopposition=288,loopsize=.5cm,lw=1,color=my_cp5_col2,opacity=0.7](E)(E);

\Edge[lw=1,color=my_cp5_col2,opacity=0.7](A)(B);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](A)(C);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](A)(D);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](A)(E);

\Edge[lw=1,color=my_cp5_col2,opacity=0.7](B)(C);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](B)(D);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](B)(E);

\Edge[lw=1,color=my_cp5_col2,opacity=0.7](C)(D);
\Edge[lw=1,color=my_cp5_col2,opacity=0.7](C)(E);

\Edge[lw=1,color=my_cp5_col2,opacity=0.7](D)(E);





%%------------------------------------------
%%------------ Graph 2 -----------------------
%%------------------------------------------

% Offset to locate the graphs

\path (plot2.south)+(0, -4*\my_gap_inter_plots)  coordinate (caux1);	


%----------- Drawing the nodes ------------

\SetDefaultUnit{pt}

% radius underlying circle = 2cm
\def\myrad{2cm};

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=1, opacity=0.7,fontsize=\Large]{A}

\path (caux1)++(0.3090*\myrad ,0.9511*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=2, opacity=0.7,fontsize=\Large]{B}

\path (caux1)++(-0.8090*\myrad , 0.5878*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=3, opacity=0.7,fontsize=\Large]{C}

\path (caux1)++(-0.8090*\myrad,-0.5878*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=4, opacity=0.7,fontsize=\Large]{D}

\path (caux1)++(0.3090*\myrad,-0.9511*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=4, opacity=0.7,fontsize=\Large]{E}

%----------- Drawing the Edges  ------------

\Edge[loopposition=0,loopsize=.5cm,lw=1,color=my_cp5_col5,opacity=0.7](A)(A);
\Edge[loopposition=72,loopsize=.5cm,lw=1,color=my_cp5_col5,opacity=0.7](B)(B);
\Edge[loopposition=144,loopsize=.5cm,lw=1,color=my_cp5_col5,opacity=0.7](C)(C);
\Edge[loopposition=216,loopsize=.5cm,lw=1,color=my_cp5_col5,opacity=0.7](D)(D);
\Edge[loopposition=288,loopsize=.5cm,lw=1,color=my_cp5_col5,opacity=0.7](E)(E);

\Edge[lw=1,color=my_cp5_col5,opacity=0.7](A)(B);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](A)(C);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](A)(D);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](A)(E);

\Edge[lw=1,color=my_cp5_col5,opacity=0.7](B)(C);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](B)(D);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](B)(E);

\Edge[lw=1,color=my_cp5_col5,opacity=0.7](C)(D);
\Edge[lw=1,color=my_cp5_col5,opacity=0.7](C)(E);

\Edge[lw=1,color=my_cp5_col5,opacity=0.7](D)(E);








%%------------------------------------------
%%------------ Graph 3 -----------------------
%%------------------------------------------

% Offset to locate the graphs

\path (plot3.south)+(0, -4*\my_gap_inter_plots)  coordinate (caux1);	


%----------- Drawing the nodes ------------

\SetDefaultUnit{pt}

% radius underlying circle = 2cm
\def\myrad{2cm};

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=1, opacity=0.7,fontsize=\Large]{A}

\path (caux1)++(0.3090*\myrad ,0.9511*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=2, opacity=0.7,fontsize=\Large]{B}

\path (caux1)++(-0.8090*\myrad , 0.5878*\myrad )  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=3, opacity=0.7,fontsize=\Large]{C}

\path (caux1)++(-0.8090*\myrad,-0.5878*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=4, opacity=0.7,fontsize=\Large]{D}

\path (caux1)++(0.3090*\myrad,-0.9511*\myrad)  coordinate (caux2);	
\gettikzy{(caux2)}{\ay};	
\gettikzx{(caux2)}{\ax};	
\Vertex[x=\ax, y=\ay, style={color=my_cp5_col3},size=\mynodesize,label=4, opacity=0.7,fontsize=\Large]{E}

%----------- Drawing the Edges  ------------

\Edge[loopposition=0,loopsize=.5cm,lw=1,color=my_cp5_col3,opacity=0.7](A)(A);
\Edge[loopposition=72,loopsize=.5cm,lw=1,color=my_cp5_col3,opacity=0.7](B)(B);
\Edge[loopposition=144,loopsize=.5cm,lw=1,color=my_cp5_col3,opacity=0.7](C)(C);
\Edge[loopposition=216,loopsize=.5cm,lw=1,color=my_cp5_col3,opacity=0.7](D)(D);
\Edge[loopposition=288,loopsize=.5cm,lw=1,color=my_cp5_col3,opacity=0.7](E)(E);

\Edge[lw=1,color=my_cp5_col3,opacity=0.7](A)(B);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](A)(C);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](A)(D);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](A)(E);

\Edge[lw=1,color=my_cp5_col3,opacity=0.7](B)(C);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](B)(D);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](B)(E);

\Edge[lw=1,color=my_cp5_col3,opacity=0.7](C)(D);
\Edge[lw=1,color=my_cp5_col3,opacity=0.7](C)(E);

\Edge[lw=1,color=my_cp5_col3,opacity=0.7](D)(E);





	
\end{tikzpicture}










==> v13/sec_discussion.tex <==
\subsection{Discussion}

==> v13/sec_gandgraphonSP.tex <==
 %!TEX root =../compiler_paper.tex



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%  SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Graph and Graphon Signal Processing}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%  Sub-Section   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Graph signal processing}

Let $G=(V(G),E(G),w_{G})$ be a graph with a set of vertices $V(G)$, a set of edges $E(G)$ and a weight function $w: E(G)\rightarrow\mathbb{R}^{+}$. A signal on the graph $G$ is defined as the map $\bbf:V(G)\rightarrow\mathbb{R}$. The images of $\bbf$ are associated to vectors in $\mathbb{R}^{N}$ where $N=\vert V(G)\vert$. The characteristics of $G$ are in general embedded in the adjacency matrix $\mathbf{A}$ whose entries are given by $\mathbf{A}(i,j) = w(\{i,j\})$ with $\{i,j\}\in E(G)$, and the degree matrix $\mathbf{D}$ whose entries are given by $\mathbf{D}(i,j)=0\quad\forall\quad i\neq j$ and $\mathbf{D}(i,i)=\sum_{j=1}^{N}\bbA(i,j)$. From $\mathbf{A}$ and $\mathbf{D}$ it is possible to define several \textit{shift operators} that serve as building blocks for the graph signal processing (GSP) machinery. Among such operators are $\bbA$ and the Laplacian operator. For a graph $G$ the shift operator will be denoted by $\bbS_G$. In our discussion we consider that $\bbS_G = \bbA$.

With the clear definition of $\bbS_G$ we define convolutional filters as matrix polynomials, i.e. a graph filter $\bbH(\bbS_G )$ can be written as
%
%
%
\begin{equation}
\bbH (\bbS_G)
                   =
                   \sum_{k=0}^{K}h_{k}\bbS^{k}_G
                   ,
\end{equation}
%
%
% 
and it acts on a graph signal $\bbf$ according to 
%
%
%
$
\bbH (\bbS)\bbf
=
\sum_{k=0}^{K}h_{k}\bbS^{k}_G\bbf
.
$
%
%
%
If $\bbS_G$ is diagonalizable, we have $\mathbf{S}_G =\mathbf{U}\mathbf{\Lambda}\mathbf{U}^{\mathsf{T}}$, where $\bbU$ is an orthogonal matrix and $\mathbf{\Lambda}$ its a diagonal matrix containing the eigenvalues of $\bbS_G$. We can calculate the \textit{graph Fourier transform} (GFT) of a signal $\bbf$ as $\hat{\bbf}=\mathbf{U}^{\mathsf{T}}\bbf$. The $i$th component in $\hat{\bbf}$ is associated to the eigenvalue $\lambda_{i}(G)$, $\mathbf{\Lambda}(i,i) = \lambda_{i}(G)$, and $\mathbf{\Lambda}(i,j)=0~\forall~ i\neq j$. In this paper the ordering of the $\lambda_{i}( \bbS_G )$'s is given by $\vert\lambda_{1}(\bbS_G )\vert\geq\vert\lambda_{2}(\bbS_G)\vert \geq\cdots\geq\vert\lambda_{N}(\bbS_G)\vert$. A graph signal $\bbf$ is said to be bandlimited with bandwidth $\omega$ if $\hat{\bbf}(i) = 0$ for all $\lambda_i (\bbS_G) < \omega$. The set of bandlimited signals with bandwidth $\omega$ is denoted by $\mathcal{PW}_{\omega}(G)$. To avoid confusions when comparing signals associated to different graphs we use the notation $(\bbf , G)$ to make emphasis on the fact that $\bbf$ is defined on $G$.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%  Sub-Section   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Graphon signal processing}


%%%------------------------------------------------------
%%%------------------- FIGURE ---------------------------
%%%------------------------------------------------------
%
%\begin{figure}
%	\includegraphics[width=1\columnwidth]{./figures/fig_1_standalone.pdf}
%	\caption{Three different discretization strategies to build graphs from a graphon. Left: a regular grid defines a set of sub domains that whose area defines the weights of the adjacency matrix. Center: an irregular grid defines a set of non uniform subdomains whose area defines the entries of the adjacency matrix. Right: The entries of the adjacency matrix are obtained directly as specific values of the graphon at a certain number of points.}
%	\label{fig_graphon_to_graph}
%\end{figure}
%
%%%---------------- End of Figure -----------------------



Graphs can be also modeled in the context of \textit{graphons}~\cite{lovasz2012large,Diao2016ModelfreeCO} when sequences of graphs are analyzed. A graphon is a symmetric measurable function $W: [0,1]^{2}\rightarrow [0,1]$ that can play the role of a \textit{limit} for some sequences of graphs~\cite{lovasz2012large}. The connection stated between the graphon and the graphs in the sequence can be obtained by means of different types of \textit{discretization} or \textit{sampling} of the graphon. Some of the main strategies for this discretization are the following:


\begin{itemize}
%
%
\item (\textbf{GD1}) Building a \textbf{regular} grid on $[0,1]^{2}$ and associating the area of the graphon $W(x,y)$ in each subdomain of the grid to a given entry in an adjacency matrix $\mathbf{A}$ (see Fig.~\ref{fig_graphon_to_graph}(left)).
%
%
\item (GD-2) Building an \textbf{irregular} grid on $[0,1]^{2}$ and associating the area of the graphon $W(x,y)$ in each subdomain of the grid to a given entry in an adjacency matrix $\mathbf{A}$ (see Fig.~\ref{fig_graphon_to_graph}(center)).
%
%
\item (GD-3) Obtaining the entries of an adjacency matrix $\mathbf{A}$ \textbf{sampling} its values from $W(x,y)$ (see Fig.~\ref{fig_graphon_to_graph}(right)).
%
%
\end{itemize}


As pointed out in~\cite{lovasz2012large,Diao2016ModelfreeCO}, given a graph $G=(V(G),E(G),w)$ with adjacency matrix $\bbA$ it is possible to obtain an \textit{induced} graphon $W_{G}$ building a uniform (regular) partition of $[0,1]$ with $N=\vert V(G)\vert$ intervals $I_{i}$ such that
%
%
%
\begin{equation}
W_{G}(u,v) =
                   \sum_{i,j=1}^{N}\bbA (i,j)\chi_{I_{i}}(u)\chi_{I_{j}}(v)
,
\end{equation}
%
%
%
where $\chi_{I_{i}}(u)$ is given by
%
%
%
\begin{equation}
\chi_{I_{i}}(u) = 
                         \begin{cases}
                                    1,\quad \text{if}\quad u\in I_i \\
                                    0,\quad \text{otherwise}
                         \end{cases}
                         .
\end{equation}
%
%
%
%Notice that the functions $\chi_{I_{i}}(u)$ constitute a basis for $\ccalP_N$ as a vector space. 

Given the relationship between a graph $G$ and its induced graphon representation, a signal $\bbf$ on $G$ induces a signal $\boldsymbol{f}$ on $W_{G}$ whose relationship with $\bbf$ is given by
%
%
%
\begin{equation}
\boldsymbol{f}(t)=\sum_{i=1}^{N} \mathbf{f}(i)\chi_{I_{i}}(t)
,
\end{equation}
%
%
%
with $t\in [0,1]$. Then, given a graphon $W_{G}$ induced by the graph $G$, it is possible to say that the set of piecewise constant functions -- according to the $I_{i}$'s -- is uniquely identified with the signals on the graph. In order to state this connection in a formal way and for the analysis in subsequent sections, we consider the notation introduced in the following definition.




%%-------------------------------------------
%%--------------- Definition--------------------
%%-------------------------------------------

\begin{definition}\label{def_PN}
Given a partition of the interval $[0,1]$ into $N$ intervals $I_{i}$, we define the set of piecewise constant functions with resolution $N$ by
%
%
%
\begin{equation}
\mathcal{P}_{N}=
                           \left\lbrace 
                                                \left.  
                                                    \boldsymbol{f}(t)\in L^{2}[0,1] 
                                                \right\vert 
                                                     \boldsymbol{f}(t_{1})=\boldsymbol{f}(t_2) ~\forall~ t_1, t_2\in I_{i}
                           \right\rbrace
                           .
\end{equation}
%
%
%
\end{definition}

%%------------- End of Definition----------------



From definition~\ref{def_PN} we can see that the extension of signals on a graph $G$ to the induced graphon $W_{G}$ can be done mapping the graph signal $\mathbf{f}$ to an element of $\mathcal{P}_{N}$ where $N=\vert N(G)\vert$. Notice that $\mathcal{P}_{N}$ is a vector space whose basis functions are $\chi_{I_{i}}(t)$. 

For our discussion it is also useful to consider spaces $\mathcal{P}_{N}$ with different values of $N$ that can be related by the partition intervals associated to each space. In the following definition we introduce the terminology used to this end. 



%%-------------------------------------------
%%--------------- Definition--------------------
%%-------------------------------------------

\begin{definition}	
Let $\mathcal{P}_{N_1}$ and $\mathcal{P}_{N_2}$ with $N_{2}>N_{1}$ be two spaces of piecewise constant functions. Let $I_{i}^{(\ell)}$ the intervals in the partition of $[0,1]$ associated to $\mathcal{P}_{N_\ell}$. Then, we say that $\mathcal{P}_{N_1}$ and $\mathcal{P}_{N_2}$ are \textbf{nested} if $I_{i}^{(1)}=\bigcup_{j\in\mathcal{J}}I_{j}^{(2)}$, where $\mathcal{J}\subset \{ 1,\ldots,N_2 \}$.
\end{definition}

%%------------- End of Definition----------------



It is worth pointing out that when two spaces $\ccalP_{N_1}$ and $\ccalP_{N_2}$ are nested with $N_2 > N_1$, we have that $\ccalP_{N_1}\subset \ccalP_{N_2}$. These notion will allow us to relate signals on graphons and graphs with different number of nodes but that are part of a sequence.


For an arbitrary graphon $W(x,y)$ -- not necessarily induced by a graph --, a signal $\boldsymbol{f}$ on $W(x,y)$ is a function $\boldsymbol{f}(t): [0,1] \rightarrow \mbR$ in $L^2 ([0,1])$. We point out that a graphon signal is a \textit{node level statistic} in the sense defined in~\cite{Diao2016ModelfreeCO}.



As mentioned in~\cite{lovasz2012large} every graphon $W$ can be used to define a Hilbert-Schmit operator that allows the study of properties of $W$, but additionally it can be used as a building block operator for the analysis of information defined on graphons~\cite{Diao2016ModelfreeCO}. Given $W$ a \textit{graphon operator} $\boldsymbol{T}_{W}$ acting on the graphon signal $(\boldsymbol{x},W)$ is given by

%
%
%
\begin{equation}\label{eq_Tw}
\left(\boldsymbol{T}_{W}\boldsymbol{x}\right)(u)
                   =
                       \int_{0}^{1}W(u,v)\boldsymbol{x}(v)dv.
\end{equation}
%
%
%

Similar to the graph signals scenarios, we need to leverage a \textit{graphon shift operator} to define the notion of filtering. For a graphon $W(u,v)$ the graphon shift operator will be denoted by $\boldsymbol{S}_W$ and it will be assumed to be $\boldsymbol{S}_W = \boldsymbol{T}_W$. Then, a convolutional filter $\boldsymbol{H}(\boldsymbol{S}_{W})$ on a graphon $W(x,y)$ is given by the polynomial operator
%
%
%
\begin{equation}
\boldsymbol{H}(\boldsymbol{S}_{W})
                         =
                           \sum_{k=0}^{K}h_{k}\boldsymbol{S}_{W}^{k}
                          , 
\end{equation}
%
%
%
where $\boldsymbol{S}_{W}^{k}$ indicates the $k$-times composition of the operator $\boldsymbol{S}_{W}$,
and whose action on the graphon signal $(\boldsymbol{x},W)$ is given by 
%
%
%
$
\boldsymbol{H}(\boldsymbol{S}_{W})\boldsymbol{x}
=
\sum_{k=0}^{q}h_{k}\boldsymbol{S}_{W}^{k}\boldsymbol{x} 
.
$
%
%
%
Then, given the relationship between graphs and their induced graphons we translate filtering from one domain to the other. In particular, for a given filter $\mathbf{H}(\mathbf{S}_G )=\sum_{k=0}^{q}h_{k}\mathbf{S}^{k}_G$ operating on signals defined on a graph $G$ it is possible to associate the graphon filter $\boldsymbol{H}(\boldsymbol{S}_{W_{G}})=\sum_{k=0}^{q}h_{k}\boldsymbol{S}_{W_{G}}^{k}$ acting on functions defined on $W_{G}$.


If the eigenvalues of $\boldsymbol{S}_W$ are countable -- which is the case when $\boldsymbol{S}_W = \boldsymbol{T}_W$ --, it is possible to obtain a Fourier decomposition of the graphon signals. Then, if $\lambda_{i}(\boldsymbol{S}_W)$ and $\boldsymbol{u}_{W,i}$ are the eigenvalues and the eigenvectors of $\boldsymbol{S}_{W}$, respectively, we can have a representation of a graphon signal $(\boldsymbol{x}, W)$ as
%
%
%
\begin{multline}
\boldsymbol{x} 
            =
               \sum_{i=1}^{\infty}\hat{\boldsymbol{x}}\left(
                                                                                           i
                                                                                   \right)
                                                                                   \boldsymbol{u}_{W,i}(t),
\quad\quad
\hat{\boldsymbol{x}}(j)=\int_{0}^{1}\boldsymbol{x}(t)\boldsymbol{u}_{W,j}(t)dt
,
\end{multline}
%
%
%
where the discrete function $\hat{\boldsymbol{x}}$ is called the \textit{graphon Fourier transform} (WFT) of $\boldsymbol{x}$. The ordering of the eigenvalues $\lambda_{i}(\boldsymbol{S}_W)$ is given by $\vert\lambda_{1}(\boldsymbol{S}_W)\vert\geq\vert\lambda_{2}(\boldsymbol{S}_W)\vert\geq\cdots$. We say that a graphon signal $\boldsymbol{x}$ is bandlimited with bandwidth $\omega$ if $\hat{\boldsymbol{x}}(i) = 0$ for all $\vert\lambda_{i}(\boldsymbol{S}_W)\vert<\omega$. The set of graphon bandlimited signals with bandwidth $\omega$ is represented by $\mathcal{PW}_{\omega}(W)$.


% Note that if $W_G$ is induced by $G$, we have $\lambda_i(\bbS_W) = \lambda_i (G)/N$ for $i=1,\ldots, N$ and $\lambda_i(\bbT_W) = 0$ for all $i>N$~\cite{lovasz2012large,Diao2016ModelfreeCO}. Additionally, if $\bbv_i$ is the $i$-th eigenvector of $\bbS$ -- the shift operator associated to the graph $G$ --, the $i$-th eigenvector of $\bbT_{W}$ is given by $\boldsymbol{\varphi}_i (t) =\sqrt{N}\sum_{\ell=1}^{N}\chi_{I_\ell}(t)\bbv_i (\ell)$~\cite{gao2019graphon}(p. 19-20).













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% Sub-Section %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{GSP convergence to WSP}

We mentioned before that graphons can be considered as limit objects of sequences of graphs whose number of nodes and edges grows to infinity. In this section we make these statements more precise, and to do so we need to introduce the notion of homomorphisms between graphs. A homomorphism between two graphs $G_1 = (V(G_1), E(G_1), w_{G_1})$ and $(G_2,V(G_2),w_{G_2})$ is a map between nodes that preserves the adjacency relationship. Then, the map $\alpha: V(G_1) \rightarrow V(G_2)$ is a homomorphism if $\{  \alpha(i), \alpha(j) \} \in E(G_2)$ if $\{ i, j \} \in E(G_1)$. Denoting by $\mathsf{hom}(G_1,G_2)$ the number of homomorphisms between $G_1$ and $G_2$ a density of homomorphisms can be defined as $t(G_1 , G_2) = \mathsf{hom}(G_1 , G_2)/\vert V(G_2) \vert^{\vert V(G_2)\vert}$. Analogously, we can consider densities of homomorphisms between a graph $G$ and a graphon $W(x,y)$ as
%
%
%
\begin{equation}
t(G , W)
               = 
                     \int_{[0,1]^{\vert V(G)\vert}} 
                                \prod_{\{ i, j\} \in E(G) } W(x_i , x_j)dx_1 \ldots dx_{\vert V(G) \vert} 
                                .
\end{equation}
%
%
%
As shown in~\cite{lovasz2012large,Diao2016ModelfreeCO}, if $W_{G_2}$ is the graphon induced by $G_2$ it follows that $t(G_1,W_{G_2}) = t(G_1 , G_2)$. With these notions at hand we say that given a fix graph $H = (V(H),E(H),w_{H})$, the sequence of graphs $\{ G_i \}_{i=0}^{\infty}$ converges to the graphon $W(x,y)$ if $\lim_{i\rightarrow\infty}t(H,G_i) = t(H,W)$ for all simple finite graphs $H$. This will be noted by $\{  G_i \}_i \rightarrow W(x,y)$. This notion of convergence is compatible with another notion of convergence in the $\delta_{\square}(\cdot,\cdot)$ metric. As proven in~\cite{lovasz2012large,Diao2016ModelfreeCO}, if $\{ G_i \} \rightarrow W(x,y)$ in the homomorphism density, then $\delta_{\square}(W_{G_i}, W)\rightarrow 0$, where
%
%
%
\begin{equation}
\delta_{\square}(W_{G_i}, W) = 
                          \inf_{\pi}
                          \left\Vert 
                                    W
                                    -
                                    \pi(W_{G_i})
                          \right\Vert_{\square} 
                          ,
\end{equation}
%
%
%
$\pi: [0,1]\rightarrow [0,1]$ is a measure preserving map acting on $W_{G_i}(x,y)$ according to $\pi (W_{G_i}(x,y)) = W_{G_i}(\pi(x),\pi(y))$, and 
%
%
%
\begin{equation}
\left\Vert 
                  W(x,y)
\right\Vert_{\square}
                =
                   \sup_{I,J\subset [0,1] } 
                    \left\vert 
                                      \int_{I\times J} W(x,y) dxdy
                    \right\vert
                    .
\end{equation}
%
%
%
Notice that particular instantiations of the measure preserving map $\pi$ lead can lead to graphons that can be obtained from graphs that are obtained by label permuations of $G_i$~\cite{Diao2016ModelfreeCO}. Notice that the notion of convergence in the metric $\delta_{\square}(\cdot,\cdot)$, naturally include sequences of graphons converging to a graphon $\{ W_i (x,y) \}_i \rightarrow W(x,y)$.

In order to understand how signals on sequences of graphs or graphons are related with signals on a graphon limit, we restrict our attention to those signals that follow a notion of convergence. In particular, when analyzing sequences of graphon signals $(W_i, \boldsymbol{x}_i)$ we focus in those $\{ \boldsymbol{x}_i \}_i$ that are convergent in $L^{1}([0,1])$. This is called in~\cite{Diao2016ModelfreeCO} a \textit{continuous node-level statistic}. Then, we say that the sequence of graphon signals $(W_i,\boldsymbol{x}_i)$ converges to $(W, \boldsymbol{x})$ if $W_i \rightarrow W$ and $\Vert \boldsymbol{x}_i -\boldsymbol{x}\Vert_{L_1}\rightarrow 0$. 

%The convergence of graph sequences to graphons discussed above have implications on the spectral domain. To show this, we introduce a theorem adapted from~\cite{Diao2016ModelfreeCO}.
%
%
%%%--------------------------------------------
%%%---------------- THEOREM -------------------
%%%--------------------------------------------
%
%\begin{theorem}[5.6~\cite{Diao2016ModelfreeCO}]\label{thm_con_eigen}
%
%Let $\{ W_i (x,y) \}_i \rightarrow W(x,y)$. Suppose $\Vert W_{i} -W \Vert_{\square}\rightarrow 0$ as $i\rightarrow\infty$. For $k\geq 1$ let $P_{k}(W_i):L^{2}([0,1])\rightarrow L^{2}([0,1])$ denotes the projection on the eigenscpace of $W_i$ associated to the eigenvalues $\{  \lambda_{k}(W_i) , - \lambda_{k}(W_i) \}$. Then, for all $k\geq 1$,
%%
%%
%%
%\begin{enumerate}
%	%
%	%
%	\item $\displaystyle \lambda_{k}(W_i)\rightarrow \lambda_{k}(W)$ as $i\rightarrow\infty$,
%	%
%	% 
%	\item $\displaystyle\left\Vert P_{k}(W_i) - P_{k}(W) \right\Vert_{\ccalB (L^{2}([0,1]))} \rightarrow 0$,
%	%
%	%
%\end{enumerate}
%%
%%
%%	
%where $\Vert T \Vert_{\ccalB (L^{2}([0,1]))} = \sup_{\Vert f \Vert}\Vert Tf\Vert_{2}$.		
%\end{theorem}
%
%%%-------------- End of Theorem -----------------
%
%Theorem~\ref{thm_con_eigen} implies that the graphon Fourier decomposition of signals in a sequence indeed converge to the graphon Fourier decomposition in the limit, this is if $(W_i, \boldsymbol{x})\rightarrow (W,\boldsymbol{x})$ then $(W_i,\hat{\boldsymbol{x}}_i)\rightarrow (W, \hat{\boldsymbol{x}})$.












%%%------------------------------------------------------
%%%------------------- FIGURE ---------------------------
%%%------------------------------------------------------
%
%\begin{figure}
%\includegraphics[width=1\columnwidth]{./figures/fig4.pdf}
%\caption{Regular grids of different sizes used to generate graphs from a graphon $W(x,y)$ by means of discretization method GD-2.}
%\label{fig:discGraphon}
%\end{figure}
%
%%%---------------- End of Figure -----------------------






 

==> v13/sec_graphonSP.tex <==
%%
%%----------------Title-------------------


==> v13/sec_lambdasets.tex <==
%!TEX root =../compiler_paper.tex




%%
%%------------------------------Title----------------------------------
%%-----------------------------Section--------------------------------------------
%%
\section{$\Lambda-$removable sets in Sequences of dense Graphs}
-Here commetns about the properties: compactness characteristics and so on. Here We can put the theorem that if there is a point in the space $(\alpha_{1},\alpha_{2},\ldots)$ in the space of determinant functions with $K$ variables then there is an open ball that contains that point and so on...


%%---------------------------------Theorem-------------------------------------
%%
\begin{theorem}[Bernstein Inequality]
Let $(\boldsymbol{x},W)$ a graphon bandlimited signal with bandwidth $\omega$, then
\begin{equation}
\left\Vert \mathbf{T}\boldsymbol{x}\right\Vert\geq\omega\Vert\boldsymbol{x}\Vert
\end{equation}
\end{theorem}
\begin{proof}
See Appendix
\end{proof}




%Finite graphs can be obtained from graphons in multiple ways. For instance, as described in Section \ref{sec:graphon} and depicted in the third diagram of Figure \ref{fig:graphfromgraphon}, an $N$-node graph $G=(V(G),E(G),\alpha)$ can be \textit{sampled} from the graphon by using a function $\rho: V(G)\rightarrow [0,1]$ to map each node $i\in V(G)$ to a number $\rho(i)\in [0,1]$, such that, for any two nodes $i,j\in V(G)$, we have $\{i,j\}\in E(G)$ and $\alpha(\{i,j\})=W(\rho(i),\rho(j))$. Another possibility is to generate graphs through \textit{piece-wise approximations}, as pictured in the two left diagrams of Figure \ref{fig:graphfromgraphon}. In this case, the weight of the edge $(i,j)$ is given by
%%calculated by integrating $W(u,v)$ in $[\rho(i),\rho(i+1)]\times [\rho(j),\rho(j+1)]$, that is,
%%%%%%%%%%%%%%%%%
%\begin{equation} \label{eqn:integration}
%\alpha(\{i,j\})=\frac{1}{\Delta}\int_{\rho(j)}^{\rho(j+1)}\int_{\rho(i)}^{\rho(i+1)}W(u,v)dudv
%\end{equation}
%%%%%%%%%%%%%%%%%
%for $1<i,j<N$, where $\Delta=(\rho(i+1)-\rho(i))(\rho(j+1)-\rho(j))$ and $\rho(i)\leq\rho(i+1)$ for all $i$.




%%---------------------------------Definition-------------------------------------
%%
\begin{definition}
Let $W_{G}$ a graphon induced by a graph  $G=(V(G),E(G),\alpha)$ by means of a regular partition on $W$, where 
\begin{equation} \label{eqn:integration}
\alpha(\{i,j\})=\frac{1}{\Delta}\int_{\rho(j)}^{\rho(j+1)}\int_{\rho(i)}^{\rho(i+1)}W(u,v)dudv
\end{equation}
Then, the set of piecewise constant functions on $W_{G}$ will be denoted by $\mathcal{PC}(W_{G})$.
\end{definition}





%%---------------------------------Definition-------------------------------------
%%
\begin{definition}
Considering the class of piecewise constant functions defined on the graphon $W_{G}$ induced by the graph $G=(V,E)$ we say that a set of intervals $I_{j}$ is $\Lambda$-removable if
\begin{equation}
\left\Vert\mathbf{T}\boldsymbol{x}\right\Vert<\Lambda\Vert\boldsymbol{x}\Vert
\end{equation}
for all piecewise constant signals whose support is given by $\cup_{j}I_{j}$.
\end{definition}


%%---------------------------------Theorem----------------------------------------
%%
\begin{theorem}
If $S=\cup_{j=1}I_{j}$ is a $\Lambda-$removable set of intervals for $\mathcal{PC}(W_{G})$, then the set of intervals $S^{c}=[0,1]\setminus S$ is a uniqueness set for all the signals in $PW_{\omega}(W_{G})\cap\mathcal{PC}(W_{G})$ with $\omega>\Lambda$ 
\end{theorem}





\subsection{Uniqueness sets conditions}
Here we can extend Bernstein inequality and so on to prove that the removable sets in Graphons also lead to a concept of a unique representation. 


\subsection{Sistematic Calculation}
Maybe adaptation of Anis method and other approaches. For instance in anis we will be deleting (making zero), some parts of the graphon and with that Graphon we will calculate the operator norm and then repeat the process to keep deleting patches of the graphon until we get a decent set that can be considered a uniqueness set

